Towards Instance-Optimal Private Query Release

We study efficient mechanisms for the query release problem in differential privacy: given a workload of $m$ statistical queries, output approximate answers to the queries while satisfying the constraints of differential privacy. In particular, we are interested in mechanisms that optimally adapt to the given workload. Building on the projection mechanism of Nikolov, Talwar, and Zhang, and using the ideas behind Dudley's chaining inequality, we propose new efficient algorithms for the query release problem, and prove that they achieve optimal sample complexity for the given workload (up to constant factors, in certain parameter regimes) with respect to the class of mechanisms that satisfy concentrated differential privacy. We also give variants of our algorithms that satisfy local differential privacy, and prove that they also achieve optimal sample complexity among all local sequentially interactive private mechanisms.

==> lb.tex <==
\section{Packing Lower Bounds}
\label{sect:lb}

The starting point for the proof of Theorem~\ref{thm:lb} is the
following theorem bounding the mutual information between the input
and the output distribution of a mechanism satisfying CDP.
\begin{theorem}[\cite{BunS16}]\label{thm:mut-info-lb}
  Let $\alg$ be a mechanism satisfying $\rho$-zCDP, and let $\db$ be a
  random $n$-element database. Then,
  \[
  I(\db; \alg(\db)) \le \log_2(e) \rho n^2.
  \]
\end{theorem}

Theorem~\ref{thm:mut-info-lb} and a standard packing argument give our
main lemma.

\begin{lemma}\label{lm:packing}
  For any finite $\uni \subseteq [0,1]^m$ and every $\alpha, \rho > 0$, we have
\begin{align}
  %\label{eq:lb}
  \samp^2_\rho(\uni, \alpha) &\ge \Omega \left(\frac{1}{\sqrt{\rho}} \cdot \sqrt{\log(\sep(\uni, 4\alpha))}\right);\\
  %\label{eq:lb-infy}
  \samp_\rho^\infty(\quer, \alpha) &\ge \Omega \left(\frac{1}{\sqrt{\rho}} \cdot  \sqrt{\log(\sep_\infty(\uni), 4\alpha)}\right).
\end{align}
\end{lemma}
\begin{proof}
  We give the argument for average error; the one for worst-case error
  proceeds analogously.  
  
  Take $T$ to be a $4\alpha$-separated subset of $\uni$ achieving
  $\sep(\uni, 4\alpha)$.  Take $\db$ to be a random database generated
  by picking a uniformly random element $\row \in T$, and defining
  $\db$ to be the database consisting of $n$ copies of $\row$. If
  $\alg$ is such that $\err^2(\quer, \alg, n) \le \alpha$, then for
  any $\db$, by Markov's ineuqality we have that, with probability at
  least $3/4$, $\|\alg(\db) - \bar{\db}\|_2 \le 2\alpha^2
  \sqrt{m}$. Let $y$ be the closest point in $T$ to $\alg(\db)$ in
  Euclidean norm. Since any two elements $\row, \row'$ of $T$ satisfy
  $\|\row - \row'\|_2 > 4\alpha \sqrt{m}$, we have that, with
  probability at least $3/4$, $y = x$. By Fano's inequality,
  \[
  I(\db; \alg(\db)) > \frac34 \log_2(|T| - 1) - 1.
  \]
  The lower bound now follows from Theorem~\ref{thm:mut-info-lb}. 
\end{proof}

Theorem~\ref{thm:lb} is a direct consequence of Lemma~\ref{lm:packing}
and the following well-known inequality, which follows by a padding
argument (see~\cite{BunUV14}):
\begin{align*}
  %\label{eq:padding}
  \forall t \ge \alpha: \ \ 
  &\samp^2_\rho(\uni, t) \le \lceil\frac{\alpha}{t}\rceil \cdot
  \samp^2_\rho(\uni, t); \\
  &\samp^\infty_\rho(\uni, t) \le \lceil\frac{\alpha}{t}\rceil \cdot
  \samp^\infty_\rho(\uni, t). 
\end{align*}


